What is the Best Automated Metric for Text to Motion Generation?

There is growing interest in generating skeleton-based human motions from natural language descriptions. While most efforts have focused on developing better neural architectures for this task, there has been no significant work on determining the proper evaluation metric. Human evaluation is the ultimate accuracy measure for this task, and automated metrics should correlate well with human quality judgments. Since descriptions are compatible with many motions, determining the right metric is critical for evaluating and designing effective generative models. This paper systematically studies which metrics best align with human evaluations and proposes new metrics that align even better. Our findings indicate that none of the metrics currently used for this task show even a moderate correlation with human judgments on a sample level. However, for assessing average model performance, commonly used metrics such as R-Precision and less-used coordinate errors show strong correlations. Additionally, several recently developed metrics are not recommended due to their low correlation compared to alternatives. We also introduce a novel metric based on a multimodal BERT-like model, MoBERT, which offers strongly human-correlated sample-level evaluations while maintaining near-perfect model-level correlation. Our results demonstrate that this new metric exhibits extensive benefits over all current alternatives.

==> 08_supporting.tex <==
\section{Supplemental Material}

\subsection{Human Evaluation Full Descriptions}

\textit{Naturalness} descriptions, as provided to the annotators, were:


\begin{itemize}
    \item \textbf{Very Unnatural}: Does not maintain a human body shape. 
Majorly glides without taking any appropriate actions such as walking or jumping. 
Possess very jerky movements.
    \item \textbf{Unnatural}: Maintains a mostly human body shape but moves unnaturally. 
Glides moderately without taking any appropriate actions such as walking or jumping. 
Possess some jerky movements.
    \item \textbf{Neutral}: Possess some amount of gliding without taking appropriate actions such as walking or jumping. 
Moves its limbs or body in ways that are not humanly likely but are possible.
    \item \textbf{Realistic}: Possess very slight amounts of gliding without taking appropriate actions such as walking or jumping. 
Moves its limbs or body in a slightly rigid fashion.
    \item \textbf{Very Realistic}: Always moves in a human like way. 
Does not move without taking appropriate actions such as walking or jumping.
\end{itemize}


\textit{Faithfulness} descriptions were:

\begin{itemize}
    \item \textbf{Dose Not Describe}: Completely different motion which corresponds in no way to the given description.
    \item \textbf{Slightly Describes}: Has very slight resemblance to the given description (such as standing up when it describing walking) but otherwise does not correspond with the given description
    \item \textbf{Moderately Describes}: Follows the description moderately, but deviates from it in significant ways such as adding major actions or leaving out a portion of the description.
    \item \textbf{Greatly Describes}: Leaves out minor details of the description or includes minor unmentioned actions. 
For example, the person may be walking as mentioned in the description but also doing actions with their hands that were unmentioned.
    \item \textbf{Perfectly Describes}: Perfectly described by the description, with no actions left out or incorrectly included.
\end{itemize}




\subsection{Model Level Comparisons}

\begin{figure}
\centering
\includegraphics[width=\linewidth]{resources/mean_rating_stats.png}
\caption{Mean rating scores from human judgment for each model utilized (including ground truth). As expected, ground truth achieves a slight lead. Note that these results are not conclusive for evaluating the capabilities of these models, as the sample sizes are relatively small and do not accurately account for a stochastic generation. }
\label{fig:by-model-mean-ratings}
\end{figure}

The primary goal of this study was not to compare the performance differences between the baseline models included. Consequently, we did not take measures to ensure that our collected data would constitute a suitably valid sample set for assessing the overall performance of each model. This is due to two main reasons: insufficient sample size and inadequate repetitions per sample. To make our study comparable, at the model level, to the evaluations conducted in each work's independent studies, we would need to evaluate the entire HumanML3D test set. Moreover, we would need to execute multiple (typically 10) generation repetitions per sample for models with stochastic generative properties. However, our study did not fulfill these requirements.

Keeping these caveats in mind, we present the mean distributions of human judgments for each of the baseline models in Figure \ref{fig:by-model-mean-ratings}. As anticipated, the ground-truth motions in the HumanML3D dataset exhibit a clear advantage in terms of \textit{Naturalness}. Their lead in \textit{Faithfulness} is less pronounced when compared to the best-performing generative baselines, \cite{DBLP:conf/eccv/GuoZWC22} and \cite{DBLP:journals/corr/abs-2208-15001}. This might indicate quality limitations in the ground-truth descriptions of the HumanML3D dataset, which were human-annotated, and qualitative analysis revealed some poor descriptions.

Another intriguing observation is the minimal observed performance difference between the two leading generative baseline models \cite{DBLP:conf/eccv/GuoZWC22} and \cite{DBLP:journals/corr/abs-2208-15001}, despite MotionDiffuse reporting gains in R-Precision, FID, and Multimodal Distance over \cite{DBLP:conf/eccv/GuoZWC22}. These findings may stem from the model coverage limitations we discussed earlier. Alternatively, they could arise from noise in our human judgment ratings or be indicative of the imperfect correlation of these metrics observed in our study.

\subsection{Evaluation Hyperparameters}

Our evaluation involved several hyperparameters, which are listed below. Whenever possible, we utilized pre-existing code, such as the evaluation script that implements FID, R-Precision, and Multimodal Distance from \cite{https://doi.org/10.48550/arxiv.2209.14916}. R-Precision employed the standard batch size of 32. For CE metrics, we searched root scalings ranging from $2^{-15}$ to $2^{14}$ in factors of 2. When combining position, velocity, and acceleration components for CE metrics, we performed a grid search to explore all possible combinations of component scalings from $2^{0}$ to $2^{9}$.

\subsection{Baseline Model Selection}

In selecting the text-conditioned motion generation models to include in our study, our primary focus was to obtain a diverse sampling of motions, as each model may be prone to its own distributional differences. However, we also imposed additional constraints on the models studied to ensure their relevance.

Although several older models exist that could potentially increase the diversity of our motion samples, we excluded them due to their subpar performance, which renders the diversity less valuable for future models. Studying these less effective models might be interesting, but their inclusion could compromise our findings by reducing the number of samples we could incorporate for better-performing models and possibly leading to a false impression of which metric is most suitable for them.

The models included in our study were also required to be compatible with and have pretrained weights available for motion generation using 22 joint SMPL body models. Some models that might have performed well enough to be considered relevant for our study cannot use 22 joint SMPL body models and would, therefore, be unsuitable for scoring against 22 joint reference motions or with 22 joint-based motion encoders.

\subsection{Metrics for Motion Diversity}
The increasing popularity of FID, Multimodal Distance, and R-Precision metrics has led to a growing interest in the metric of Diversity, proposed alongside them. However, in this study, we did not examine Diversity for several reasons. Measuring diversity necessitates a distinct experimental setup compared to others, as multiple generations for a single prompt are required. Furthermore, there is no well-defined method for assessing diversity from a human perspective. Current metrics evaluate the diversity of embedded representations, but it remains unclear how annotators should be instructed to measure diversity. A separate study should investigate measures of diversity, their alignment with human judgments, and the impact of enhancing a model's diversity of outputs on its \textit{Faithfulness} and \textit{Naturalness} judgments.


\subsection{Supplemental Data}
Our code can be found on the following repository: 

We provide all collected human motion judgments for both \textit{Naturalness} and \textit{Faithfulness} as supplemental data to this work. Additionally, we include the prompts used to generate each motion sample and the motion generations themselves. Our data zip files contain the following files and formats:

\begin{itemize}
\item ratings\_and\_captions.csv: A comma-separated file with each line containing, in order; restricted sample index, model name, original sample index, the mean value for the sample for human judgment of Naturalness, the mean value for the sample for human judgment of Faithfulness, and the lowercase textual prompt it corresponds with/was generated from. The model names are either HumanML3D, MotionDiffuse, text2motion, TM2T, or MDM. The original sample index is the index from a larger superset of 400 samples for each model, which were initially included in the human annotation collection. After quality control and restricting to samples with valid judgments across all baseline models, this number was reduced to 280 samples per model, as indicated by the restricted sample index.
\item AMASS\_motion\_{ModelName}\_{SampleIndex}.npy: The motion sequences utilized in this study, each in AMASS format for a 22 Joint SMPL body model. All other joints have zeroed out values. The value SampleIndex in the file name corresponds with the original sample index value from the ratings\_and\_captions.csv file.
\end{itemize}

We anticipate that this data and code will be valuable for reproducing our results and facilitating future testing of innovative text-conditioned motion generation metrics.


\subsection{Loss Functions and Human Judgement Optimization}
Certain generative models for human motions employ loss functions that resemble the CE metrics we evaluated, such as Pose POS AE. The moderate correlation with human judgments observed in our study raises questions about the advisability of this approach. We propose that higher-scoring differentiable metrics might be more effective. Even non-differentiable metrics, like NNC metrics, could be incorporated into the learning process through reinforcement learning. This method could optimize highly-correlated metrics and potentially lead to improved human-judged performance.

\subsection{MoBERT Regression Model Hyperparameters}
We utilize Sklearn's SVR and Ridge classes for learning a regression head with human guidance. For the SVR model we utilize the following Sklearn parameters: kernel='rbg', gamma='scale', coef0=0.0, tol=1e-8, C=3.68, epsilon=0.3, and shrinking=False. For the Linear Ridge model we utilize the following Sklearn parameters: alpha=0.12, fit\_intercept=True, max\_iter=6, tol=1e-3, solver='saga', and positive=False. For the Ridge model we utilize a learned Sklearn StandardScalar in the pipeline of our regression model to normalize output embedding of our Transformer Encoder. The full model architectures, include which output embedding features are utilized, are shown in Figures \ref{fig:svr-model} and \ref{fig:ridge-model}. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{resources/svr_model.png}
    \caption{Our MoBERT evaluation pipeline with a RBF SVR regression head. Max indicates a per-dimension max operation was utilize to aggregate the grouped embeddings. }
    \label{fig:svr-model}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{resources/ridge_model.png}
    \caption{Our MoBERT evaluation pipeline with a Linear Ridge regression head. Max indicates a per-dimension max operation was utilize to aggregate the grouped embeddings. }
    \label{fig:ridge-model}
\end{figure}

\subsection{MoBERT as a Text-Free Naturalness Evaluator}

\begin{table*}
\begin{center}
\begin{tabular}{|| l r | c | c | c | c ||} 
 \hline
 %\multicolumn{6}{|| c ||}{Pearson Correlation with Human Judgements} \\
   & & \multicolumn{2}{| c |}{Model Level} & \multicolumn{2}{| c ||}{Sample Level} \\
  \cline{3-6}
  \multicolumn{2}{|| c |}{Metric} & Faithfulness & Naturalness & Faithfulness & Naturalness \\[0.5ex]
  \hline\hline
 MoBERT Score (Alignment Probability) & $\uparrow$ & \textbf{0.991} & 0.841 & 0.488 & 0.324 \\
 MoBERT Score (SVR Regression)* & $\uparrow$ & 0.962 & \textbf{0.986} & \textbf{0.624} & \textbf{0.528} \\
 MoBERT Score (Linear Regression)* & $\uparrow$ & 0.951 & 0.975 & 0.608 & 0.515 \\
 MoBERT Text-Free Score (Alignment Probability) & $\uparrow$ & 0.036 & 0.575 & -0.048 & -0.031 \\
 MoBERT Text-Free Score (SVR Regression)* & $\uparrow$ & 0.935 & 0.871 & 0.399 & 0.483 \\
 MoBERT Text-Free Score (Linear Regression)* & $\uparrow$ & 0.928 & 0.804 & 0.383 & 0.468 \\
\hline
\end{tabular}
\end{center}
\caption{Pearson correlations with human judgments calculated for MoBERT with and without text. The best-performing metric in each category is bolded. Models with (*) were judged through 10-fold cross-validation. Arrows next to metrics indicate whether negative ($\downarrow$) or positive ($\uparrow$) correlation is expected. }
\label{fig:results-corrs-tf}
\end{table*}

MoBERT employs a Faithfulness-centered task in its training, with Alignment Prediction effectively serving as a binary predictor for the Faithfulness of the motion-text pair. However, the model has not encountered situations lacking text, which we investigate in this ablation. We aim to derive multiple insights from this exploration.

Initially, we treated Naturalness as an autonomous factor during our human judgment dataset collection, independent of text. However, the interpretation of Naturalness is context-sensitive. For instance, a directive such as "a person performing a wild and crazy dance" might seem unnatural out of context, yet within its particular context, it could appear somewhat natural. Our model may learn to consider this context, so examining the model's behavior in absence of the text is an effective probe for which features it learns to consider.

Moreover, a text-free Naturalness evaluator may be advantageous in certain circumstances. While MoBERT, in comparison to other metrics like FID/CE, does not demand reference motions or large sample sizes like R-Precision/FID, it still requires a valid text description, limiting its flexibility. This ablation demonstrates how effectively MoBERT performs in scenarios where no reference information is available, in the form of either text or motions.

Additionally, this ablation provides a sanity check on our model's results. Although we anticipate that the textual context will enhance the judgment of Naturalness, a too significant difference might suggest text overfitting rather than the identification of useful features in the motion's Naturalness. In contrast, a significant drop in Faithfulness is expected as it should theoretically be impossible to judge the Faithfulness of a motion without its associated descriptions, thus probing the model's operation. However, we predict that the learned regressors will still achieve some correlation with Faithfulness, as Faithfulness strongly correlates with Naturalness which is predictable. Hence, a well-trained regressor could base its Faithfulness scores on features used to judge Naturalness. We predict a score lower than the text-free correlation for Naturalness, but above $62\%$ of it, considering the observed 0.62 correlation between Faithfulness and Naturalness.

Table \ref{fig:results-corrs-tf} presents our ablation findings. As anticipated, our hypotheses are confirmed. The sample-level correlation scores for Naturalness marginally decrease by about 0.045 with the loss of context, while Faithfulness experiences a more substantial drop of 0.225 Pearson's, yet remains above $62\%$ of the Naturalness correlation result. Furthermore, the raw Alignment Probability approaches zero for both quality types, suggesting the additional regression training is needed to identify output features suitable for text-free evaluation. These results not only affirm MoBERT's ability to learn diverse and beneficial features, but they also prove its capacity to operate as a text-free Naturalness evaluator, surpassing the sample-level correlations of all other non-MoBERT metrics, even those requiring reference motions or text.


\subsection{MoBERT Full Architecture}
Our complete MoBERT model architecture, output from PyTorch 2.0, is presented below. Note our alignment prediction head does not include the Sigmoid layer as it is trained using the PyTorch BCEWithLogitsLoss method. 
\begin{verbatim}

(word_embs): Embedding(2000, 256)
(pos_embs): Embedding(64, 256)
(seq_embs): Embedding(2, 256)

(frame_encoder): Sequential(
  (0): Linear(
    in_features=263, 
    out_features=384, 
    bias=True
  )
  (1): GroupNorm(8, 384, eps=1e-05, affine=True)
  (2): SELU()
  (3): Dropout(p=0.2, inplace=False)
  (4): Linear(
    in_features=384, 
    out_features=384, 
    bias=True
  )
  (5): GroupNorm(8, 384, eps=1e-05, affine=True)
  (6): SELU()
  (7): Dropout(p=0.2, inplace=False)
)

(chunk_encoder): Sequential(
  (0): Linear(
    in_features=5376, 
    out_features=5376, 
    bias=True
  )
  (1): GroupNorm(14, 5376, eps=1e-05, affine=True)
  (2): SELU()
  (3): Dropout(p=0.2, inplace=False)
  (4): Linear(
    in_features=5376, 
    out_features=1792, 
    bias=True
  )
  (5): GroupNorm(8, 1792, eps=1e-05, affine=True)
  (6): SELU()
  (7): Dropout(p=0.2, inplace=False)
  (8): Linear(
    in_features=1792, 
    out_features=1024, 
    bias=True
  )
  (9): GroupNorm(8, 1024, eps=1e-05, affine=True)
  (10): SELU()
  (11): Dropout(p=0.2, inplace=False)
  (12): Linear(
    in_features=1024, 
    out_features=256, 
    bias=True
  )
  (13): GroupNorm(8, 256, eps=1e-05, affine=True)
  (14): SELU()
  (15): Dropout(p=0.2, inplace=False)
)

(transformer_encoder): TransformerEncoder(
  (layers): ModuleList(
    (0-2): 3 x TransformerEncoderLayer(
      (self_attn): MultiheadAttention(
        (out_proj): NonDynamicallyQuantizableLinear(
          in_features=256, 
          out_features=256, 
          bias=True
        )
      )
      (linear1): Linear(
        in_features=256, 
        out_features=1024, 
        bias=True
      )
      (dropout): Dropout(p=0.1, inplace=False)
      (linear2): Linear(
        in_features=1024, 
        out_features=256, 
        bias=True
      )
      (norm1): LayerNorm((256,), 
        eps=1e-05, 
        elementwise_affine=True
      )
      (norm2): LayerNorm((256,), 
        eps=1e-05, 
        elementwise_affine=True
      )
      (dropout1): Dropout(p=0.1, inplace=False)
      (dropout2): Dropout(p=0.1, inplace=False)
    )
  )
)

(alignment_pred_head): Sequential(
  (0): Linear(
    in_features=256, 
    out_features=128, 
    bias=True
  )
  (1): GroupNorm(8, 128, eps=1e-05, affine=True)
  (2): SELU()
  (3): Dropout(p=0.2, inplace=False)
  (4): Linear(
    in_features=128, 
    out_features=128, 
    bias=True
  )
  (5): GroupNorm(8, 128, eps=1e-05, affine=True)
  (6): SELU()
  (7): Dropout(p=0.2, inplace=False)
  (8): Linear(
    in_features=128, 
    out_features=1, 
    bias=True
  )
)

\end{verbatim}


\subsection{Statistical Significance}

Our correlation results yielded high P-Values at both the sample and model levels, not including our MoBERT model which obtained near zero P-Values. High P-Values at the sample level are expected due to the low correlations, which increase the likelihood of the null hypothesis. For the model level results, despite observing higher correlations, the limited sample size contributes to elevated P-Values. Examining model level results reduces our dataset to only five samples, making spurious correlations more likely by random chance and increasing P-Values.

In this section (Figures \ref{fig:p-val1} - \ref{fig:p-val7}), we present the same graphs from the main paper, but with added grey bars indicating P-Value. Notably, our most recommended metrics achieve relatively low P-Values, near or below the desired 0.05 threshold.

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{resources/correlation_of_fid_score_with_human_ratings_w_pvalue.png}
    \caption{Model level FID correlations with human judgments. Grey bars indicate the P-Values achieved for the correlations. }
    \label{fig:p-val1}
\end{figure*}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{resources/human_ratings_and_ae_individual_samples_w_pvalue.png}
    \caption{Sample level AE correlations with human judgments. Grey bars indicate the P-Values achieved for the correlations.}
    \label{fig:p-val2}
\end{figure*}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{resources/human_ratings_and_ae_model_average_w_pvalue.png}
    \caption{Model level AE correlations with human judgments. Grey bars indicate the P-Values achieved for the correlations.}
    \label{fig:p-val3}
\end{figure*}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{resources/human_ratings_and_ave_individual_samples_w_pvalue.png}
    \caption{Sample level AVE correlations with human judgments. Grey bars indicate the P-Values achieved for the correlations.}
    \label{fig:p-val4}
\end{figure*}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{resources/human_ratings_and_ave_model_average_w_pvalue.png}
    \caption{Model level AVE correlations with human judgments. Grey bars indicate the P-Values achieved for the correlations.}
    \label{fig:p-val5}
\end{figure*}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{resources/r_precision_correlation_across_retrieval_allowance_individual_samples_w_pvalue.png}
    \caption{Sample level R-Precision correlations with human judgments. Grey bars indicate the P-Values achieved for the correlations.}
    \label{fig:p-val6}
\end{figure*}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{resources/r_precision_correlation_across_retrieval_allowance_model_average_w_pvalue.png}
    \caption{Model level R-Precision correlations with human judgments. Grey bars indicate the P-Values achieved for the correlations.}
    \label{fig:p-val7}
\end{figure*}
